Pansharpening by convolutional neural networks in the full resolution framework

In recent years, there has been a growing interest in deep learning-based pansharpening. Thus far, research has mainly focused on architectures. Nonetheless, model training is an equally important issue. A first problem is the absence of ground truths, unavoidable in pansharpening. This is often addressed by training networks in a reduced resolution domain and using the original data as ground truth, relying on an implicit scale invariance assumption. However, on full resolution images results are often disappointing, suggesting such invariance not to hold. A further problem is the scarcity of training data, which causes a limited generalization ability and a poor performance on off-training test images. In this paper, we propose a full-resolution training framework for deep learning-based pansharpening. The framework is fully general and can be used for any deep learning-based pansharpening model. Training takes place in the high-resolution domain, relying only on the original data, thus avoiding any loss of information. To ensure spectral and spatial fidelity, a suitable two-component loss is defined. The spectral component enforces consistency between the pansharpened output and the low-resolution multispectral input. The spatial component, computed at high-resolution, maximizes the local correlation between each pansharpened band and the panchromatic input. At testing time, the target-adaptive operating modality is adopted, achieving good generalization with a limited computational overhead. Experiments carried out on WorldView-3, WorldView-2, and GeoEye-1 images show that methods trained with the proposed framework guarantee a pretty good performance in terms of both full-resolution numerical indexes and visual quality.

==> ArXiv - R3/preambol.tex <==


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\usepackage{amsmath,amsfonts,epsfig,graphicx}
\usepackage{subfig}
\usepackage{color,soul}
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{balance}
\usepackage{url}
\usepackage{multirow,hhline}
\usepackage{placeins}
\usepackage{wasysym}
\usepackage{amssymb}
\usepackage{pifont}% http://ctan.org/pkg/pifont
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\xmark}{\ding{53}}%

\usepackage[nomessages]{fp}% http://ctan.org/pkg/fp
%\captionsetup{belowskip = -5pt}


%% Z-PNN scope
\newcommand{\Lms}{\mathcal{L}_{\rm MS}}
\newcommand{\Lpan}{\mathcal{L}_{\rm PAN}}

\newcommand{\Md}{M_\downarrow}
\newcommand{\Mu}{M_\uparrow}
%\newcommand{\Xd}{X_\downarrow}
%\newcommand{\Xu}{X_\uparrow}
%\newcommand{\hXd}{\hat{X}_\downarrow}
%\newcommand{\hX}{\hat{X}}



\newcommand{\hMd}{\hat{M}_\downarrow}
\newcommand{\wMd}{\widehat{M}_\downarrow}
\newcommand{\hM}{\hat{M}}
\newcommand{\Pd}{P_\downarrow}
\newcommand{\Mdu}{M_{\downarrow\uparrow}}





%%





\newcommand{\by}{\mathbf{f}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{v}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
%\newcommand{\hM}{\hat{M}}
%\newcommand{\tM}{\widetilde{M}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\brd}{\mathbf{r}_{\downarrow}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bxd}{\mathbf{x}_{\downarrow}}
\newcommand{\bpd}{\mathbf{p}_{\downarrow}}
\newcommand{\hx}{\widehat{\mathbf{x}}}
\newcommand{\hxd}{\widehat{\mathbf{x}}_{\downarrow}}
\newcommand{\hr}{\widehat{\mathbf{r}}_{\downarrow}}
\newcommand{\hhx}{\widehat{\widehat{\mathbf{x}}}_{\downarrow}}
%
\newcommand{\tx}{\widetilde{\mathbf{x}}}
\newcommand{\txd}{\widetilde{\mathbf{x}}_{\downarrow}}
%
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bad}{\mathbf{a}_{\downarrow}}

%\DeclareMathOperator{\BN}{BN}

\newcommand{\image}{\pgfuseimage}

\newcommand{\figpath}{./Figures/}
%\newcommand{\tabpath}{./tables/}
\newcommand{\figTempPath}{./../drawing/scatterLS/}
\newcommand{\figGbPath}{./../drawing/G_beta_scatter/G_b_scatter_}




\definecolor{colPeppe}{rgb}{0.9, 0.1, 0.1}
%\newcommand{\peppe}[1]{{\color{colPeppe} #1}}
\newcommand{\peppe}[1]{{#1}}

\newcommand{\red}[1]{{\color{red} #1}}


%%%%%%%%IMAGE & TABLES%%%%%%%%%%%%%


%% Adelaide
\newcommand{\pathAdeRRplots}{./../drawing/Adelaide_RR_plots/}
\newcommand{\pathAdeFRplots}{./../drawing/Adelaide_FR_plots/}
\newcommand{\pathAdeRRcrops}{./../drawing/Adelaide_RR_crops/}
\newcommand{\pathAdeFRcrops}{./../drawing/Adelaide_FR_crops/}



%% Washington
\newcommand{\pathWashRRplots}{./../drawing/Washington_RR_plots/}
\newcommand{\pathWashFRplots}{./../drawing/Washington_FR_plots/}
\newcommand{\pathWashRRcrops}{./../drawing/Washington_RR_crops/}
\newcommand{\pathWashFRcrops}{./../drawing/Washington_FR_crops/}







\newcommand{\heiT}{4.17cm}
\newcommand{\heiB}{4.5cm}




\newcommand{\ru}{\rule{0mm}{3mm}}

%%%%%%%%%%%%%%%% LABELS %%%%%%%%%%%%%%%
\newcommand{\labsty}[1]{{\scriptsize #1}}
\newcommand{\labSty}[1]{{#1}}

\newcommand{\labGT}{\labSty{Ground-truth}}
\newcommand{\labMS}{\labSty{MS}}
\newcommand{\labPAN}{\labSty{PAN}}
\newcommand{\labProp}{\labSty{Proposed}}
\newcommand{\labPnn}{\labSty{A-PNN}}
\newcommand{\labDrpnn}{\labSty{DRPNN}}
\newcommand{\labPannet}{\labSty{PanNet}}
\newcommand{\labGLP}{\labSty{MTF-GLP-HPM}}
\newcommand{\labATWT}{\labSty{ATWT-M3}}
\newcommand{\labAWLP}{\labSty{AWLP}}
\newcommand{\labBDSD}{\labSty{BDSD}}
\newcommand{\labCBDSD}{\labSty{C-BDSD}}
\newcommand{\labCBDSDF}{\labSty{C-BDSD-Fast}}
\newcommand{\labPRACS}{\labSty{PRACS}}
\newcommand{\labEXP}{\labSty{EXP}}
\newcommand{\labGSA}{\labSty{GSA}}
\newcommand{\labINDUSION}{\labSty{Indusion}}
\newcommand{\labGLPCBD}{\labSty{MTF-GLP-CBD}}


\newcommand{\LabGT}{\labsty{Ground-truth}}
\newcommand{\LabMS}{\labsty{MS}}
\newcommand{\LabPAN}{\labsty{PAN}}
\newcommand{\LabProp}{\labsty{Proposed}}
\newcommand{\LabPnn}{\labsty{A-PNN}}
\newcommand{\LabDrpnn}{\labsty{DRPNN}}
\newcommand{\LabPannet}{\labsty{PanNet}}
\newcommand{\LabGLP}{\labsty{MTF-GLP-HPM}}
\newcommand{\LabATWT}{\labsty{ATWT-M3}}
\newcommand{\LabAWLP}{\labsty{AWLP}}
\newcommand{\LabBDSD}{\labsty{BDSD}}
\newcommand{\LabCBDSD}{\labsty{C-BDSD}}
\newcommand{\LabCBDSDF}{\labsty{C-BDSD-Fast}}
\newcommand{\LabPRACS}{\labsty{PRACS}}
\newcommand{\LabEXP}{\labsty{EXP}}
\newcommand{\LabGSA}{\labsty{GSA}}
\newcommand{\LabINDUSION}{\labsty{Indusion}}
\newcommand{\LabGLPCBD}{\labsty{MTF-GLP-CBD}}







%\newcommand{\labQNR}{\labsty{QNR}}
%\newcommand{\labDs}{\labsty{D$_s$}}
%\newcommand{\labDl}{\labsty{D$_\lambda$}}
%\newcommand{\labQq}{\labsty{Q4}}
%\newcommand{\labQ}{\labsty{Q}}
%\newcommand{\labERGAS}{\labsty{ERGAS}}
%\newcommand{\labSAM}{\labsty{SAM}}

\newcommand{\labQNR}{\textbf{QNR}}
\newcommand{\labDs}{\textbf{D$_{S}$}}
\newcommand{\labDl}{\textbf{D$_{\lambda}$}}
\newcommand{\labQq}{\textbf{Q4}}
\newcommand{\labQo}{\textbf{Q8}}
\newcommand{\labQ}{\textbf{Q}}
\newcommand{\labERGAS}{\textbf{ERGAS}}
\newcommand{\labSAM}{\textbf{SAM}}

\newcommand{\labCPU}{\labSty{CPU}}
\newcommand{\labGPU}{\labSty{GPU}}







\DeclareMathOperator{\CC}{CC}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\decimation}{Dec}
\DeclareMathOperator{\SAM}{SAM}
\DeclareMathOperator{\ERGAS}{ERGAS}
\DeclareMathOperator{\RMSE}{RMSE}
\DeclareMathOperator{\HQNR}{HQNR}


\newcommand{\DL}{D_{\lambda}^{(\rm K)}}
\newcommand{\DS}{D_{\rm S}}
\newcommand{\DR}{D_{\rho}}














==> preambol.tex <==


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\usepackage{amsmath,amsfonts,epsfig,graphicx}
\usepackage{subfig}
\usepackage{color,soul}
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{balance}
\usepackage{url}
\usepackage{multirow,hhline}
\usepackage{placeins}
\usepackage{wasysym}
\usepackage{amssymb}
\usepackage{pifont}% http://ctan.org/pkg/pifont
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\xmark}{\ding{53}}%

\usepackage[nomessages]{fp}% http://ctan.org/pkg/fp
%\captionsetup{belowskip = -5pt}


%% Z-PNN scope
\newcommand{\Lms}{\mathcal{L}_{\rm MS}}
\newcommand{\Lpan}{\mathcal{L}_{\rm PAN}}

\newcommand{\Md}{M_\downarrow}
\newcommand{\Mu}{M_\uparrow}
%\newcommand{\Xd}{X_\downarrow}
%\newcommand{\Xu}{X_\uparrow}
%\newcommand{\hXd}{\hat{X}_\downarrow}
%\newcommand{\hX}{\hat{X}}



\newcommand{\hMd}{\hat{M}_\downarrow}
\newcommand{\wMd}{\widehat{M}_\downarrow}
\newcommand{\hM}{\hat{M}}
\newcommand{\Pd}{P_\downarrow}
\newcommand{\Mdu}{M_{\downarrow\uparrow}}





%%





\newcommand{\by}{\mathbf{f}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{v}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
%\newcommand{\hM}{\hat{M}}
%\newcommand{\tM}{\widetilde{M}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\brd}{\mathbf{r}_{\downarrow}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bxd}{\mathbf{x}_{\downarrow}}
\newcommand{\bpd}{\mathbf{p}_{\downarrow}}
\newcommand{\hx}{\widehat{\mathbf{x}}}
\newcommand{\hxd}{\widehat{\mathbf{x}}_{\downarrow}}
\newcommand{\hr}{\widehat{\mathbf{r}}_{\downarrow}}
\newcommand{\hhx}{\widehat{\widehat{\mathbf{x}}}_{\downarrow}}
%
\newcommand{\tx}{\widetilde{\mathbf{x}}}
\newcommand{\txd}{\widetilde{\mathbf{x}}_{\downarrow}}
%
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bad}{\mathbf{a}_{\downarrow}}

%\DeclareMathOperator{\BN}{BN}

\newcommand{\image}{\pgfuseimage}

\newcommand{\figpath}{./Figures/}
%\newcommand{\tabpath}{./tables/}
\newcommand{\figTempPath}{./../drawing/scatterLS/}
\newcommand{\figGbPath}{./../drawing/G_beta_scatter/G_b_scatter_}




\definecolor{colPeppe}{rgb}{0.9, 0.1, 0.1}
%\newcommand{\peppe}[1]{{\color{colPeppe} #1}}
\newcommand{\peppe}[1]{{#1}}

\newcommand{\red}[1]{{\color{red} #1}}


%%%%%%%%IMAGE & TABLES%%%%%%%%%%%%%


%% Adelaide
\newcommand{\pathAdeRRplots}{./../drawing/Adelaide_RR_plots/}
\newcommand{\pathAdeFRplots}{./../drawing/Adelaide_FR_plots/}
\newcommand{\pathAdeRRcrops}{./../drawing/Adelaide_RR_crops/}
\newcommand{\pathAdeFRcrops}{./../drawing/Adelaide_FR_crops/}



%% Washington
\newcommand{\pathWashRRplots}{./../drawing/Washington_RR_plots/}
\newcommand{\pathWashFRplots}{./../drawing/Washington_FR_plots/}
\newcommand{\pathWashRRcrops}{./../drawing/Washington_RR_crops/}
\newcommand{\pathWashFRcrops}{./../drawing/Washington_FR_crops/}







\newcommand{\heiT}{4.17cm}
\newcommand{\heiB}{4.5cm}




\newcommand{\ru}{\rule{0mm}{3mm}}

%%%%%%%%%%%%%%%% LABELS %%%%%%%%%%%%%%%
\newcommand{\labsty}[1]{{\scriptsize #1}}
\newcommand{\labSty}[1]{{#1}}

\newcommand{\labGT}{\labSty{Ground-truth}}
\newcommand{\labMS}{\labSty{MS}}
\newcommand{\labPAN}{\labSty{PAN}}
\newcommand{\labProp}{\labSty{Proposed}}
\newcommand{\labPnn}{\labSty{A-PNN}}
\newcommand{\labDrpnn}{\labSty{DRPNN}}
\newcommand{\labPannet}{\labSty{PanNet}}
\newcommand{\labGLP}{\labSty{MTF-GLP-HPM}}
\newcommand{\labATWT}{\labSty{ATWT-M3}}
\newcommand{\labAWLP}{\labSty{AWLP}}
\newcommand{\labBDSD}{\labSty{BDSD}}
\newcommand{\labCBDSD}{\labSty{C-BDSD}}
\newcommand{\labCBDSDF}{\labSty{C-BDSD-Fast}}
\newcommand{\labPRACS}{\labSty{PRACS}}
\newcommand{\labEXP}{\labSty{EXP}}
\newcommand{\labGSA}{\labSty{GSA}}
\newcommand{\labINDUSION}{\labSty{Indusion}}
\newcommand{\labGLPCBD}{\labSty{MTF-GLP-CBD}}


\newcommand{\LabGT}{\labsty{Ground-truth}}
\newcommand{\LabMS}{\labsty{MS}}
\newcommand{\LabPAN}{\labsty{PAN}}
\newcommand{\LabProp}{\labsty{Proposed}}
\newcommand{\LabPnn}{\labsty{A-PNN}}
\newcommand{\LabDrpnn}{\labsty{DRPNN}}
\newcommand{\LabPannet}{\labsty{PanNet}}
\newcommand{\LabGLP}{\labsty{MTF-GLP-HPM}}
\newcommand{\LabATWT}{\labsty{ATWT-M3}}
\newcommand{\LabAWLP}{\labsty{AWLP}}
\newcommand{\LabBDSD}{\labsty{BDSD}}
\newcommand{\LabCBDSD}{\labsty{C-BDSD}}
\newcommand{\LabCBDSDF}{\labsty{C-BDSD-Fast}}
\newcommand{\LabPRACS}{\labsty{PRACS}}
\newcommand{\LabEXP}{\labsty{EXP}}
\newcommand{\LabGSA}{\labsty{GSA}}
\newcommand{\LabINDUSION}{\labsty{Indusion}}
\newcommand{\LabGLPCBD}{\labsty{MTF-GLP-CBD}}







%\newcommand{\labQNR}{\labsty{QNR}}
%\newcommand{\labDs}{\labsty{D$_s$}}
%\newcommand{\labDl}{\labsty{D$_\lambda$}}
%\newcommand{\labQq}{\labsty{Q4}}
%\newcommand{\labQ}{\labsty{Q}}
%\newcommand{\labERGAS}{\labsty{ERGAS}}
%\newcommand{\labSAM}{\labsty{SAM}}

\newcommand{\labQNR}{\textbf{QNR}}
\newcommand{\labDs}{\textbf{D$_{S}$}}
\newcommand{\labDl}{\textbf{D$_{\lambda}$}}
\newcommand{\labQq}{\textbf{Q4}}
\newcommand{\labQo}{\textbf{Q8}}
\newcommand{\labQ}{\textbf{Q}}
\newcommand{\labERGAS}{\textbf{ERGAS}}
\newcommand{\labSAM}{\textbf{SAM}}

\newcommand{\labCPU}{\labSty{CPU}}
\newcommand{\labGPU}{\labSty{GPU}}







\DeclareMathOperator{\CC}{CC}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\decimation}{Dec}
\DeclareMathOperator{\SAM}{SAM}
\DeclareMathOperator{\ERGAS}{ERGAS}
\DeclareMathOperator{\RMSE}{RMSE}
\DeclareMathOperator{\HQNR}{HQNR}


\newcommand{\DL}{D_{\lambda}^{(\rm K)}}
\newcommand{\DS}{D_{\rm S}}
\newcommand{\DR}{D_{\rho}}













